CoShare: An Efficient Approach for Redundancy Allocation in NFV

An appealing feature of Network Function Virtualization (NFV) is that in an NFV-based network, a network function (NF) instance may be placed at any node. On the one hand this offers great flexibility in allocation of redundant instances, but on the other hand it makes the allocation a unique and difficult challenge. One particular concern is that there is inherent correlation among nodes due to the structure of the network, thus requiring special care in this allocation. To this aim, our novel approach, called CoShare, is proposed. Firstly, its design takes into consideration the effect of network structural dependency, which might result in the unavailability of nodes of a network after failure of a node. Secondly, to efficiently make use of resources, CoShare proposes the idea of shared reservation, where multiple flows may be allowed to share the same reserved backup capacity at an NF instance. Furthermore, CoShare factors in the heterogeneity in nodes, NF instances and availability requirements of flows in the design. The results from a number of experiments conducted using realistic network topologies show that the integration of structural dependency allows meeting availability requirements for more flows compared to a baseline approach. Specifically, CoShare is able to meet diverse availability requirements in a resource-efficient manner, requiring, e.g., up to 85% in some studied cases, less resource overbuild than the baseline approach that uses the idea of dedicated reservation commonly adopted for redundancy allocation in NFV.

==> pics/2-system_model-bt-yj.tex <==
\section{The System Model and Problem Definition}\label{sec-syst}
In this section, we first present the system model, including the network model and the availability model. Then, we introduce the redundancy resource allocation problem and highlight the associated challenges. %availability requirement

\subsection{Network Model} %{Basic System Model}
\nop{
We consider network services provided by an NFV-based network to its flows. The network is represented as an undirected graph $G(\mathcal{N},\mathcal{L})$, where $\mathcal{N}$ denotes the set of nodes and $\mathcal{L}$ the set of links interconnecting the nodes. A flow $f$ has a source node ($s_f$) and a destination node ($d_f$), and is identified by the source-destination node pair ($s_f$, $d_f$). The network service provided to a flow $f$ is represented by an NF chain $\overrightarrow{S}_f$,  i.e. a set of network functions $(S^1_f, S_f^2 \ldots S_f^{g_f})$ that are performed in the specified order, where $g_f$ denotes the service chain length. The traffic rate of flow $f$ is denoted by $\lambda_f$.

A node in the network directly forwards the traffic of a flow to the next node on the decided path, if the node does not host any NF for the flow. Otherwise, the related NF instances at the node will first perform those NFs on the traffic before forwarding to the next node.  To have a complete overview of the network topology, such source and destination nodes, called ``edge'' nodes in the remainder, and the related links are included in $G(\mathcal{N},\mathcal{L})$.  

%To simply the investigation, we practically assume that the edge nodes do not have resources to host NF instances. %the {\em edge nodes are not involved in hosting NF instances} and that their effect on the network service availability is excluded. 
We practically assume that the edge nodes are not involved in hosting NF instances. A non-edge node may have multiple CPU cores to host NF instances. An NF instance can be hosted on any node that has enough available resources. Following the literature \cite{zhang2016opennetvm, woldeyohannes2018cluspr}, it is assumed that a CPU core, if allocated, is dedicated to a single NF instance. 

An NF instance of type $v$ requires $k_v$ number of cores and has $\mu_v$ processing capacity (i.e., the amount of traffic the instance can process per unit time). An NF instance may process multiple flows whose service chains include the type of NF instance. It is required that $\sum_{f \in \mathcal{F}^v} \lambda_f \leq \mu_v$, where $\mathcal{F}^v$ denotes the set of flows processed by this NF instance $v$. %The capacity of NF instance $v$ for this is denoted by $\mu_v$, and

It is assumed that each flow has already been assigned a {\em primary path} for its NF chain, which includes nodes with NF instances of the service chain, using an NFV resource allocation algorithm, e.g. ClusPR\cite{woldeyohannes2018cluspr}, where, however, the availability aspect of the service may not have been taken into particular consideration.
}
We consider network services provided by an NFV-based network to its flows. The network is represented as an undirected graph $G(\mathcal{N},\mathcal{L})$, where $\mathcal{N}$ denotes the set of nodes and $\mathcal{L}$ the set of links. %To simplify the representation and analysis, the (physical) links of the network are also considered to be vertices and included in $\mathcal{N}$. With this, the edges $\mathcal{L}$  only represent logic connections between vertices, which are hence assumed to be $100\%$-available with unlimited capacity. 
Each flow $f$ has a source ($s_f$) and a destination ($d_f$), and is identified by the source-destination pair ($s_f$, $d_f$), where $s_f$ and $d_f$ are in $\mathcal{N}$. We call such source and destination nodes ``edge'' nodes in the remainder and practically assume that the edge nodes are not involved in hosting NF instances. A non-edge node may have multiple CPU cores to host NF instances. {\em An NF instance can be hosted on any such node that has enough available resources}. Following the literature \cite{zhang2016opennetvm, woldeyohannes2018cluspr}, it is assumed that a CPU core, if allocated, is dedicated to a single NF instance. 

The network service provided to flow $f$ is represented by an NF chain $\overrightarrow{S}_f$,  i.e. a set of network functions $(S^1_f, S_f^2 \ldots S_f^{g_f})$ that are performed in the specified order, where $g_f$ denotes the service chain length. The traffic rate of the flow is denoted by $\lambda_f$. 
A node in the network directly forwards the traffic of the flow to the next node on the decided path, if the node does not host any NF for the flow. Otherwise, the related NF instances at the node will first perform those NFs on the traffic before forwarding to the next node.  

An NF instance of type $v$ requires $k_v$ number of cores and has $\mu_v$ processing capacity (i.e., the amount of traffic the instance can process per unit time). An NF instance may process multiple flows whose service chains include this type of NF instance. It is required that $\sum_{f \in \mathcal{F}^v} \lambda_f \leq \mu_v$, where $\mathcal{F}^v$ denotes the set of flows processed by this NF instance $v$. 

It is assumed that each flow has already been assigned a {\em primary path} for its NF chain, which includes nodes with NF instances of the service chain, using an NFV resource allocation algorithm, e.g. ClusPR\cite{woldeyohannes2018cluspr}, where, however, the availability aspect of the service may not have been taken into particular consideration.


\subsection{Availability Model} %{Availability Requirement}
\nop{
In this paper, we assume that the network service provided to each flow $f$ has an availability requirement $A_f^r$, where again for practical consideration, the effect of the source and destination nodes of the flow on the network service availability is excluded. 
%Note that one may consider the edge nodes as devices of the network users. For this reason and to simply the model, we assume that the {\em edge nodes are not involved in hosting NF instances} and that their effect on the network service availability is excluded. 
We are interested in {\em meeting the availability requirements of flows by redundancy}, through placement and allocation of additional resources particularly NF instances. More specifically, if the primary NF chain path cannot provide the required $A_f^r$, {\em backup path(s)} are created to improve the availability level of the service and meet the requirement. The service to a flow is considered available if either the primary or one of the backup service chain paths is available. %$\overrightarrow{S}_f$ is

It is worth highlighting that, a backup path here is for the NF chain implementing the service. As such, this {\em NF chain backup path} not only needs to potentially carry traffic of the flow but also has to implement the NFs on the chain in the required order. Consequently, the problem differs from the classical backup path problem that involves no NF implementation, which has been studied for long time \cite{Doucette03} and for different types of networks~\cite{li2002efficient,ou2004shared-path,Tornatore:05,xu2006}. 
%particularly the impact of a node failure may have on the interruption of a network service
% Similar approaches have been proposed for path-based restoration functionality applied to MPLS, IP, and optical mesh networks~\cite{li2002efficient,ou2004shared-path,Tornatore:05,xu2006} where backup paths are shared among disjoint working paths. However, applying this concept to NFV redundancy allocation differentiates from standard shared backup-path restoration for several reasons. First, in shared-path protection approaches, the backup path selection is carried out exploiting shared risk group (SRG) concepts with apriori knowledge of the network topology~\cite{li2002efficient,ou2004shared-path,Tornatore:05,xu2006}. 

To simplify the representation, we assume that the graph $G(\mathcal{N},\mathcal{L})$ has been constructed such that 
{\em all links in the graph $G(\mathcal{N},\mathcal{L})$ are $100\%$-available with unlimited capacity}. Note that, while this perfect-link assumption seems to be unrealistic or rather restrictive, it actually is not. This is because, in $G(\mathcal{N},\mathcal{L})$, a link does not have to mean a physical link: Indeed, a physical link can be represented by a node in the graph with two ``perfect links'' connecting both sides of the physical link. 
% \footnote{This assumption seems to be rather restrictive, but actually not: Note that the links of the graph do not have to mean physical links, and a physical link can be represented as a node in the graph with two ``perfect link'' connecting both sides of the physical link}. 
In addition, we assume that node failures are independent, so are NF instance failures that are further assumed to be independent from node failures. 
}
A node or link may fail. In addition, a network function instance may also fail. To simplify the representation and analysis, we assume that all such failures are independent. 

In this paper, we suppose that the network service provided to each flow $f$ has an availability requirement $A_f^r$, where again for practical consideration, the effect of the source and destination nodes of the flow on the network service availability is excluded. 

%Note that one may consider the edge nodes as devices of the network users. For this reason and to simply the model, we assume that the {\em edge nodes are not involved in hosting NF instances} and that their effect on the network service availability is excluded. 
We are interested in {\em meeting the availability requirements of flows by redundancy}, through allocation of additional resources particularly NF instances. More specifically, if the primary NF chain path cannot provide the required $A_f^r$, {\em backup path(s)} are created to improve the availability level of the service and meet the requirement. The service to a flow is considered available if either the primary or one of the backup service chain paths is available.

%$\overrightarrow{S}_f$ is %placement and assignment
\yuming{This should be updated: Here we need to put the availability model, taking into account both node and link availability.}
Let $A_n$ denote the availability of node $n$, i.e., the probability that the node is available, and similarly $A_v$ the availability of NF instance $v$. 
For the primary NF chain path $p_{f}$ of flow $f$, we use $A^p_{f}$ to denote its availability, and $p_{f,g}$ the node $p$ on the primary path which serves flow $f$'s $g$-th NF on the chain. 

It is worth highlighting that, a backup path here is for the NF chain implementing the service. As such, this {\em NF chain backup path} not only needs to potentially carry traffic of the flow but also has to implement the NFs on the chain in the required order. However, in NFV resource allocation without considering availability, the typical focus has been on minimizing the number of needed NF instances while maximizing the utilization of each activated NF instance \cite{woldeyohannes2018cluspr}. As a result, it is likely that there are no enough remaining resources for the NF chain backup paths when taking availability into account. This implies that new NF instances need to be placed in the network, and subsequently be assigned to help create the backup paths. 
Consequently, the redundancy allocation problem in NFV differs from the classical backup allocation problem that involves no NF instance placement and assignment, which has been studied for long time \cite{Doucette03} and for different types of networks~\cite{li2002efficient,ou2004shared-path,Tornatore:05,xu2006}. 
%particularly the impact of a node failure may have on the interruption of a network service
% Similar approaches have been proposed for path-based restoration functionality applied to MPLS, IP, and optical mesh networks~\cite{li2002efficient,ou2004shared-path,Tornatore:05,xu2006} where backup paths are shared among disjoint working paths. However, applying this concept to NFV redundancy allocation differentiates from standard shared backup-path restoration for several reasons. First, in shared-path protection approaches, the backup path selection is carried out exploiting shared risk group (SRG) concepts with apriori knowledge of the network topology~\cite{li2002efficient,ou2004shared-path,Tornatore:05,xu2006}. 

%To simplify the representation, we assume that the graph $G(\mathcal{N},\mathcal{L})$ has been constructed such that {\em all links in the graph $G(\mathcal{N},\mathcal{L})$ are $100\%$-available with unlimited capacity}. Note that, while this perfect-link assumption seems to be unrealistic or rather restrictive, it actually is not. This is because, in $G(\mathcal{N},\mathcal{L})$, a link does not have to mean a physical link: Indeed, a physical link can be represented by a node in the graph with two ``perfect links'' connecting both sides of the physical link. 
% \footnote{This assumption seems to be rather restrictive, but actually not: Note that the links of the graph do not have to mean physical links, and a physical link can be represented as a node in the graph with two ``perfect link'' connecting both sides of the physical link}. 
%In addition, we assume that node failures are independent, so are NF instance failures that are further assumed to be independent from node failures. 

%Let $A_n$ denote the availability of node $n$, i.e., the probability that the node is available, and similarly $A_v$ the availability of NF instance $v$. 
%For the primary NF chain path $p_{f}$ of flow $f$, we use $A^p_{f}$ to denote its availability, and $p_{f,g}$ the node $p$ on the primary path which serves flow $f$'s $g$-th NF on the chain. 
%The probability that an NF application is available is denoted by $A_v$ and the probability that a backup node is available, i.e., backup node availability, is denoted by $A_b $. Table~\ref{table_example} summarizes the parameter notations used in the system model.


%A node $n$ is subject to failure, whose availability is denoted as $A_n$. It is assumed that node failures are independent. In addition, an NF instance $v$ may also fail, whose availability is denoted as $A_v$. It is assumed that such NF instance failures are independent from each other as well as from the nodes hosting them. 


%A service request or flow has a source node ($s_f$) and destination node ($d_f$), which are respectively used as an entry and exit point to the network services. These access nodes are a bottleneck for achieving high availability since the failure of one of them leads to a service impact to users relying on them. To avoid this, dual homing is utilized in which two access nodes are paired and one of the nodes may act as a backup for the other and vice versa.  %the same for the destination nodes.
%The service required by a flow $f$ is represented by a service chain, $\overrightarrow{S}_f=(S^1_f, S_f^2 \ldots S_f^{g_f})$, where $g_f$ is the service chain length of flow $f$. The service chain is an ordered series of network functions, where $S_f^g$ is the $g$-th NF of the chain with $g\in \{1,2,...,g_f\}$.
%The service chain is an ordered series of network functions, where $S^1_f$ is the first NF, $S_f^2$ is the second NF needed and so on.
%It is assumed that each flow $f$ has already been assigned a primary service chain path where the availability aspect may not have been considered. The whose availability is denoted by $A^p_{f}$. The variable $p_{f,g}$ indicates the primary node $p$ that is serving flow $f$'s $g$-th service. For each flow $f$, there is an availability requirement on its service $\overrightarrow{S}_f$, denoted as $A_f^r$. A service $\overrightarrow{S}_f$ is considered available if either the primary or one of the backup service chains is available. The average arrival rate, in number of packets per second (pps), of flow $f$ is represented by $\lambda_f$. % and {\color{red}$b(f)$ is the average arrival rate of packets per second, in other words a flow utilizes $b(f)$ amount of NF processing capacity. 
%A backup NF instance of type $v$ requires $k_v$ number of cores and has $\mu_v$ processing capacity (i.e., number of packets the instance can process per second). The probability that an NF application is available is denoted by $A_v$ and the probability that a backup node is available, i.e., backup node availability, is denoted by $A_b $. Table~\ref{table_example} summarizes the parameter notations used in the system model.


\subsection{Dissection of the Redundancy Allocation Problem}
%The ``de-facto'' technique for a system to achieve high availability for its services is through allocation of backup resources to compensate for the failures of primary ones~\cite{avizienis2004basic}. 
%Failure of one of the NFs of a service chain will result in the unavailability of the whole service function chain. 

While resource redundancy is the ``de-facto'' mechanism to cope with failures and to achieve high availability~\cite{avizienis2004basic}, in order to make use of the redundant or backup resources effectively and efficiently, a careful planning of redundancy allocation is mandatory. For an NFV-based network, the redundancy allocation problem involves three considerations to ensure the required service availability for each flow, which are, (1) using minimum number of backup NF instances, (2) optimally placing the backup NF instances in the network, and (3) efficiently assigning backup NF chain paths to flows. 

\nop{
\begin{itemize}
\item Using minimum number of backup NF instances
\item Optimally placing the backup NF instances %Deciding the optimal placement of backup instances in the network 
\item Efficiently assigning backup NF chain paths to flows
\end{itemize}
%First, it needs to (i) estimate the number of additional / backup NF instances needed to guarantee a certain availability requirement of each service chain request, (ii) the optimal placement (or mapping) of each of the backup instances on the network nodes, and (iii) the assignment of service chain requests to backup instances.


These aspects are entangled, which, together with the special NFV characteristic i.e. any node may host an instance of any NF type, make redundancy allocation in NFV both unique and challenging. 
An indicative optimization problem can be formulated as:
\begin{eqnarray}
\text{Given:}  && G(\mathcal{N},\mathcal{L}) \nonumber \\
\text{Minimize}_{\forall (\beta, \alpha)}  && N_v(\beta, \alpha), \qquad \forall v \in \mathcal{V}  \label{opt-problem}%\nonumber 
\\
\text{Such that} && A_f(\beta, \alpha) \ge A_f^r, \quad  \forall f \nonumber 
\end{eqnarray}
where $\beta$ and $\alpha$ respectively denote the adopted NF backup instance placement and assignment strategies, $\mathcal{V}$ the set of NFs involved in providing the services, $A_f(\beta, \alpha) $ the achieved availability for every flow $f$ under these strategies, and for simplicity, only the topology and the availability constraints are included. 
}

%\subsubsection
\textit{(1) Number of Backups:} %{Backup Instance Number} 
The number of backup / redundant NF instances depends on many factors, including the availability requirements of flows, the availability characteristics of both the nodes and the NF instances, as well as the topology of the network, where the NF instances are placed and how they are assigned to support the service chains of flows.

\yuming{This example needs to be updated, since it only considers node and instance, no effect of link.}For a simple example, when the availability requirements are stringent while nodes and/or NF instances have high failure probabilities, more than one backups may have to be allocated. 
%For example, to guarantee a carrier-grade service availability level~\cite{jiang2017overview}, it might be necessary to allocate more than one backup chains. 
%The following simple example is used to showcase this. 
Consider a flow that has a two-NF long service chain. Suppose, the flow requires a carrier-grade service availability level~\cite{jiang2017overview}: $A_{f}^{r} = 99.999\%$, the primary chain of the flow is $99\%$ available, i.e. $A^p_{f}=99\%$, and for all nodes and all NF instances, their availabilities are $99\%$ and $99.9\%$ respectively, i.e. $A_b= 99\%$ and $A_v=99.9\%$. If only one backup chain and accordingly the needed backup NF instances would be used, the best availability that can be achieved, e.g. by hosting the two backup instances, each for one NF in the chain, in a same node, would be: 
%\textit{Number of Backups:} The number of redundant NF instances depend on the physical mapping, and the availability characteristics of both the physical nodes and the virtual instances. In case network elements, like nodes or instances, have high failure probabilities, more than one backup element may have to be allocated. For example, to guarantee the high-availability level of carrier-grade services~\cite{jiang2017overview}, it might be necessary to allocate more than one backup chain. The following simple example is used to showcase this. Consider a flow that has two-service long chain. The primary chain of the flow is $99\%$ available ($A^p_{f}$) and the flow requires to be $99.999\%$ available ($A_{f}^{r}$). The backup nodes and NF applications are $99\%$ and $99.9\%$ available ($A_b$ and $A_v$), respectively. Thus, after being allocated backup instances that are hosted on the same backup node, the flow will have an availability of only:\vspace{-10pt}
\begin{eqnarray}
A_{f} & = & 1-[(1-A^p_{f}) \cdot (1-A_b \cdot A_v \cdot A_v)] 
%\nonumber \\ 
%& = & 1-[(1-0.99)\cdot(1-0.99\cdot0.999\cdot0.999)] \nonumber \\ 
%& =& 
= 0.99988 \nonumber
\end{eqnarray}
which does not meet the required $A_{f}^{r} = 99.999\%$. Thus, a second backup chain is needed. % to reach the required $99.999\%$ availability. %$1-(1-0.99*0.999*0.999)(1-0.99) = 0.99988$. i.e., $99.988\%$ available.
%However, this may result in a higher cost for the operator due to a high number of overall instances provisioned in the network.

%\subsubsection
\textit{(2) Placement of Backup Instances:} 
Similarly, the decision of the placement of backup instances is also influenced by multiple factors, including the network topology, the heterogeneities of nodes and NF instances in their capacities and availabilities, and the required service availabilities. As a highlight, backup instance placement should not only comply to anti-affinity constraints~\cite{isg2016network_resiliency} for avoiding common failure modes, but they should also take into account node's resource capabilities: Placing a backup instance in a given node may happen only if the node has sufficient resources, e.g. CPU cores, to host the backup instance.

%\subsubsection
\textit{(3) Assignment of Backup Instances:}  %Assignment of Backup Instances:}
This consideration concerns the assignment of backup instances to each flow to form backup NF service chains and their corresponding traffic paths in the network. In doing so, the assignment should be such that the flow's availability requirement is satisfied. 
%In doing so, flows need to be assigned to backup instances such that their availability requirements are satisfied. 
In addition, the flow can be assigned of backup instances only if the instances have sufficient resource capacity to accommodate the flow. Furthermore, an efficient assignment must consider also the delay of an NF chain backup path. 
%the additional delay introduced by the failover to the redundant instance. 
Such delays should be minimized or confined within an acceptable range.
%so that the SLAs are not violated. 
Last but not least, an effective flow assignment should avoid sharing risk of failure with the primary instances or service chain of the flow, i.e, the failure of any of the primary instances or their hosting nodes should have minimal impact on the backup instances or service chain backup path(s).

\subsection{The Redundancy Allocation Problem in a Nutshell}

The above discussed three considerations are entangled, which, together with the special NFV characteristic, i.e. any node may host an instance of any NF type, make redundancy allocation in NFV both unique and challenging. 

In the literature and real systems, the problem has been investigated. In various existing virtualization technologies, redundancy is provided in the form of virtual instance replicas, which are ready to takeover the service in case the primary instance fails. Typical solutions like VMware Fault Tolerance~\cite{vmware_ha} or more recent NFV state-of-art system-level frameworks~\cite{kulkarni_reinforce_2018} envision the instantiation of a {\em dedicated backup instance}, which runs {\em on a separate node}, shall the primary instance fail. However, such solutions can be resource inefficient as per each NF at least two instances (one primary and one backup) are required to ensure a certain availability level. 

To have a better overview of the problem and to achieve efficient resource utilization in redundancy allocation, we formulate it into an optimization problem as follows:
\begin{eqnarray}
\text{Given:}  && G(\mathcal{N},\mathcal{L}) \nonumber \\
\text{Minimize}_{\forall (\beta, \alpha)}  && N_v(\beta, \alpha), \qquad \forall v \in \mathcal{V}  \label{opt-problem}%\nonumber 
\\
\text{Such that} && A_f(\beta, \alpha) \ge A_f^r, \quad  \forall f \nonumber 
\end{eqnarray}
where $\beta$ and $\alpha$ respectively denote the adopted NF backup instance placement and assignment strategies, $\mathcal{V}$ the set of NFs involved in providing the services, $A_f(\beta, \alpha) $ the achieved availability for every flow $f$ under these strategies, and for simplicity, only the topology and the availability constraints are included. 

Though the formulation of the optimization problem in (\ref{opt-problem}) is only informative, without exhaustively listing all the constraints such as capacity constraints, the formidable complexity of the problem is implied. For this reason, a heuristic approach is adopted in this paper. In particular, a three-step approach, called CoShare, is proposed to respectively address the three considerations discussed in the previous subsection. Details of CoShare are introduced in Sections \ref{sec:heuristic} and \ref{assignment}. 

A novel idea of CoShare is to explicitly take into account the topological impact in the problem as highlighted in (\ref{opt-problem}). The underlying reason is that the failure of one node may cause the unreachability of other nodes if the latter ones have strong network structural dependency with the failed node. Therefore, in order to avoid the unavailability of NF backup instances induced by topologically correlated unreachability, taking care of structural dependency or correlation in backup instance placement and assignment is necessary. To this aim, the following Section \ref{sec:dependency_index} is dedicated. 
%To showcase this, consider (probably part of) a network of 11 nodes, $n_1 \to n_11$, as shown in Fig.~\ref{struct_correlation}. 


%Since the probability that multiple nodes will fail at the same time is low, redundancy allocation is commonly planned considering single node and/or single link failures~\cite{li2002efficient,hao2016optimizing}. With the consideration of single link and node failures, some flows are not susceptible to simultaneous failures. 

%For example, consider the two flows $f_{1}$ and $f_{3}$ depicted in Fig.~\ref{struct_correlation}. The flows traverse the network through completely disjoint paths, as they do not have a common node or link on their primary service path, hence they are not likely to experience service failures simultaneously. In addition, they have in common at least one NF type in their chains, i.e., $v_1$, whose backup instance can be shared by both. Therefore, these flows can share a backup NF capacity as shown in Fig.~\ref{shared_vs_dedicated_b}. In this case, only one backup instance is necessary in order to provide adequate protection to both primary instances. 

%A common challenge to all the above considerations is characterized by correlated failures which may incur due to network structural dependencies. The failure of one node may cause the unreachability of other nodes if the latter have network structural dependency with the failed node. To illustrate, failures of node $n_{9}$ in Fig.~\ref{struct_correlation} would make nodes $n_{10}$ and $n_{11}$ unreachable. Therefore, in order to avoid the unavailability of NF backup instances induced by topologically correlated failures, a careful backup instance placement is necessary. For example, the backup instance of the NF of type $v_{1}$, running on node $n_{9}$, should not be placed on nodes $n_{10}$ and $n_{11}$ since they highly depend on $n_{9}$. 

\nop{
\begin{figure}[t]
\centering
\includegraphics[width=0.85\columnwidth]{pics/shared_vs_dedicated_network}
\caption{\label{struct_correlation}Example of structural correlation.}
\vspace{-10pt}
\end{figure}
}

%In various existing virtualization technologies, redundancy is provided in the form of virtual instance replicas, which are ready to takeover the service in case the primary instance fails. Typical solutions like VMware Fault Tolerance~\cite{vmware_ha} or more recent NFV state-of-art system-level frameworks~\cite{kulkarni_reinforce_2018} envision the instantiation of a dedicated backup instance, which runs on a separate node and is kept in synchronization with the primary by logging the incoming traffic. However, such solutions can be resource inefficient as per each NF at least two instances (one primary and one backup) are required to ensure a certain availability level. We exploit the intuitive concept of NF shared reservation for significantly reducing the number of backup NF instances required to satisfy the service requests both in terms of processing capacity and availability demands. 

%In the design of CoShare, we exploit these considerations to efficiently use resources and allocate effective backup service function chains.  




%==========Commented below===========

\nop{
\begin{figure}[htb]
\centering
\includegraphics[width=0.8\columnwidth]{pics/net_service_topo}
\caption{\label{net_service_topo} Example of NFV service deployment.}
\vspace{-10pt}
\end{figure}

The considered system is a network of physical nodes and links and is represented as an undirected graph $G(\mathcal{N},\mathcal{L})$, where $\mathcal{N}$ denotes the set of nodes and $\mathcal{L}$ represents the set of links, interconnecting the nodes. In this paper, we concentrate on the NFV service level perspective where the failure of the NF software, hosting infrastructure, i.e., computing nodes where NFs are hosted on, and their inter-dependencies in terms of network connectivity may cause a service interruption. To this end, we regard the NFV service provisioning as the ability to deliver an end-to-end NFV-based service by steering traffic through an ordered set of NF instances deployed in a network topology composed by the interconnection of the hosting infrastructure. Fig.~\ref{net_service_topo} illustrates an example of a NFV-based service deployment. We regard this topology as a higher-level interconnection of the nodes hosting NFs where the topology can be imposed by specific routing policies applied in the transport network level. For example, the interconnection of two hosting nodes is realized through a specific route due to path delay/latency constraints. Nodes hosting NFs that are being utilized by the primary service chains of flows are called \textit{primary nodes}. Nodes that can be used for backup are referred to as \textit{backup nodes}. $\mathcal{B}$ denotes the set of backup nodes and $\mathcal{P}$ the set of primary nodes. 

\besmir{\underline{This doesnt look like really informative:} A node hosting backup instances can be used as a shared or dedicated backup node. A shared backup node is a node that is being used both as a primary and backup node, i.e., hosting both primary and backup NF instances for different service chains. \kk{can a shared backup node be used as a backup node for multiple primary NF instances? Your previous sentence does not imply this.} These type of nodes reserve some resources to be used as backup while hosting NFs that are utilized by the primary service chains. Dedicated backup nodes are nodes that are used only to host backup instances.}\kk{why do you care that you have 'dedicated' backup nodes that do not have a 'primary' node function??} 

The number of cores on a node $b \in \mathcal{B}$ is represented by $K^b$.


%For each of the primary nodes the subset of backup nodes that are preferred to be used as a backup are specified. These 
%nodes are picked based on the topology of the network and the availability of resources. For example, to use resources more efficiently all nodes in the network except the node itself might be used as a backup, or all nodes except those that are in the same rack might be used to  avoid the effect of dependency of failures etc

%Each flow $f$ specifies its source and destination nodes $s_f$ and $d_f$ respectively as well as its availability requirement, $A_f^r$. In addition, the flow has a service chain, $\overrightarrow{S}_f=(S^1_f, S_f^2 \ldots S_f^{g_f})$. The service chain is an ordered series of network functions, where $S^1_f$ is the first NF, $S_f^2$ is the second NF needed and so on. It is assumed that a flow is already assigned a primary service chain. The variable $p_{f,g}$ indicates the primary node $p$ that is serving flow $f$'s $g^{th}$ service. 
%A backup instance of an NF type $v$ requires $k_v$ number of cores and can be a backup to upto $C^b_v$ number of flows. 

A service request or flow has a source node ($s_f$) and destination node ($d_f$), which are respectively used as an entry and exit point to the network services. These access nodes are a bottleneck for achieving high availability since the failure of one of them leads to a service impact to users relying on them. To avoid this, dual homing is utilized in which two access nodes are paired and one of the nodes may act as a backup for the other and vice versa.  %the same for the destination nodes.
The service required by a flow $f$ is represented by a service chain, $\overrightarrow{S}_f=(S^1_f, S_f^2 \ldots S_f^{g_f})$, where $g_f$ is the service chain length of flow $f$. The service chain is an ordered series of network functions, where $S_f^g$ is the $g$-th NF of the chain with $g\in \{1,2,...,g_f\}$.
%The service chain is an ordered series of network functions, where $S^1_f$ is the first NF, $S_f^2$ is the second NF needed and so on.
It is assumed that a flow is already assigned a primary service chain whose availability is denoted by $A^p_{f}$. The variable $p_{f,g}$ indicates the primary node $p$ that is serving flow $f$'s $g$-th service. For each flow $f$, there is an availability requirement on its service $\overrightarrow{S}_f$, denoted as $A_f^r$. A service $\overrightarrow{S}_f$ is considered available if either the primary or one of the backup service chains is available. The average arrival rate, in number of packets per second (pps), of flow $f$ is represented by $\lambda_f$. % and {\color{red}$b(f)$ is the average arrival rate of packets per second, in other words a flow utilizes $b(f)$ amount of NF processing capacity. 
A backup NF instance of type $v$ requires $k_v$ number of cores and has $\mu_v$ processing capacity (i.e., number of packets the instance can process per second). The probability that an NF application is available is denoted by $A_v$ and the probability that a backup node is available, i.e., backup node availability, is denoted by $A_b $. Table~\ref{table_example} summarizes the parameter notations used in the system model.

% and can be a backup to up to $C^b_v$ number of flows.

%\besmir{What is this? + need to introduce SFC request availability requirement, node capacity notations etc. Table} . (Y:T)  b(f) is the amount of NF capacity each flow will consume, }%the amount of NF capacity that flow $f$ requires. 


\begin{table}[!t]
\renewcommand{\arraystretch}{1.3}
\caption{Mathematical notations}
\label{table_example}
\centering
\begin{tabular}{l | p{5cm}p{5cm}}
\hline
\bfseries Notation & \bfseries Definition\\
\hline\hline
Node and NF parameters \\
\hline\hline
$\mathcal{N}$ & set of nodes in a network\\
\hline
$\mathcal{L}$ & set of links in a network\\
\hline
$\mathcal{P}$ & set of primary nodes\\
\hline
$\mathcal{B}$ & set of backup nodes\\
\hline
$\mathcal{L}$ & set of links in a network\\
\hline
$K^b$ & number of cores available on backup node $b$\\
\hline
$\mu_v$ & processing capacity of instance $v$ in pps\\
\hline
$A_b$ & probability that backup node $b$ is available\\
\hline
$ \hat{\mathcal{B}}_{p}$ & set of backup nodes that have high structural correlation with node $p$\\ 
\hline
$k_v$ & number of cores needed to instantiate NF type $v$\\
\hline
%$A_v^p$ & the probability that a network function of type $v$ hosted on primary node $b$ is available\\
%\hline
$A_v$ & availability of an instance of type $v$\\
\hline\hline
Flow parameters \\
\hline\hline
$p_{f,g}$ & primary node $p$ that is serving flow $f$'s $g^{th}$ service\\
\hline
$\mathcal{P}_f$ & set of primary nodes used by flow $f$\\
\hline
$g_f$ & service chain length of flow $f$\\
\hline
$\lambda_f$ & average arrival rate of flow $f$ in pps\\
\hline
$s_f, d_f$ & source and destination nodes of flow $f$, respectively\\
\hline
$\overrightarrow{S}_f=(S^1_f, S_f^2 \ldots S_f^{g_f})$ & service chain of flow $f$\\%Where $S^1_f$ is flow $f$'s first service type.\\
\hline
$A_f$ & flow $f$ service availability\\
\hline
$A_f^r$ & flow $f$ service availability requirement\\
\hline
$A^p_{f}$ & flow $f$ primary service chain availability \\
\hline\hline
\end{tabular}
\end{table}



%The proposed algorithm is driven by novel intuitions that overcome challenges introduced by node unavailabilities due to correlated failures and inefficient resource utilization consisting in the following insights.

\subsection{The Redundancy Allocation Problem}
Failure of one of the NFs of a service chains will result in the unavailability of the whole service function chain. Resource redundancy, either in terms of physical and/or virtual resources, is a mechanism to cope with failures and provide fault-tolerance~\cite{avizienis2004basic}. However, in order for redundancy to be effective, a careful planning of resource allocations is mandatory. 

The redundancy resource allocation planning involves several considerations that network operators need to account for. A resource allocation plan needs to decide (i) the minimum necessary NF backup instances to guarantee a certain availability requirement of each service chain request, (ii) the optimal placement (or mapping) of each of the backup instances on the network nodes, and (iii) the assignment of service chain requests to backup instances.


\textit{Number of Backups:} The number of redundant NF instances depend on the physical mapping, and the availability characteristics of both the physical nodes and the virtual instances. In case network elements, like nodes or instances, have high failure probabilities, more than one backup element may have to be allocated. For example, to guarantee the high-availability level of carrier-grade services~\cite{jiang2017overview}, it might be necessary to allocate more than one backup chain. The following simple example is used to showcase this. Consider a flow that has two-service long chain. The primary chain of the flow is $99\%$ available ($A^p_{f}$) and the flow requires to be $99.999\%$ available ($A_{f}^{r}$). The backup nodes and NF applications are $99\%$ and $99.9\%$ available ($A_b$ and $A_v$), respectively. Thus, after being allocated backup instances that are hosted on the same backup node, the flow will have an availability of only:\vspace{-10pt}

\begin{equation}
\begin{split}
A_{f} & =1-[(1-A^p_{f}) \cdot (1-A_b \cdot A_v \cdot A_v)] \\ 
& =1-[(1-0.99)\cdot(1-0.99\cdot0.999\cdot0.999)] \\ 
& =0.99988 \nonumber
\end{split}
\end{equation}

Thus, a second backup chain is needed to reach the required $99.999\%$ availability. %$1-(1-0.99*0.999*0.999)(1-0.99) = 0.99988$. i.e., $99.988\%$ available.
However, this may result in a higher cost for the operator due to a high number of overall instances provisioned in the network.

\textit{Placement of Backup Instances:} The decision of the placement of backup instances is influenced by several factors including the heterogeneity of nodes, NF instances, and service chain requests availabilities. In addition, backup instance placement should not only comply to anti-affinity constraints~\cite{isg2016network_resiliency} for avoiding common failure modes, but they should also take into account node physical resource capabilities. Placing a backup instance in a given node may happen only if the node resource capacity is sufficient to host the backup instance.

\textit{Assignment of Backup Instances:} This consideration concerns the assignment of flows to backup instances. In doing so, flows need to be assigned to backup instances such that flow availability requirements are satisfied. Moreover, a given flow needs to be assigned to backup instances only if the instances have the sufficient resource capacity to accommodate the flow. Furthermore, an efficient assignment must consider also the additional delay introduced by the failover to the redundant instance. Such delays should be minimized or confined within an acceptable range so that the SLAs are not violated. Last but not least, an effective flow assignment should avoid sharing risk of failure with the primary instances of the flow, i.e, the failure of any of the primary instances or their hosting nodes should not affect the backup instances.


%Since the probability that multiple nodes will fail at the same time is low, redundancy allocation is commonly planned considering single node and/or single link failures~\cite{li2002efficient,hao2016optimizing}. With the consideration of single link and node failures, some flows are not susceptible to simultaneous failures. 


%For example, consider the two flows $f_{1}$ and $f_{3}$ depicted in Fig.~\ref{struct_correlation}. The flows traverse the network through completely disjoint paths, as they do not have a common node or link on their primary service path, hence they are not likely to experience service failures simultaneously. In addition, they have in common at least one NF type in their chains, i.e., $v_1$, whose backup instance can be shared by both. Therefore, these flows can share a backup NF capacity as shown in Fig.~\ref{shared_vs_dedicated_b}. In this case, only one backup instance is necessary in order to provide adequate protection to both primary instances. 
A common challenge to all the above considerations is characterized by correlated failures which may incur due to network structural dependencies. The failure of one node may cause the unreachability of other nodes if the latter have network structural dependency with the failed node. To illustrate, failures of node $n_{9}$ in Fig.~\ref{struct_correlation} would make nodes $n_{10}$ and $n_{11}$ unreachable. Therefore, in order to avoid the unavailability of NF backup instances induced by topologically correlated failures, a careful backup instance placement is necessary. For example, the backup instance of the NF of type $v_{1}$, running on node $n_{9}$, should not be placed on nodes $n_{10}$ and $n_{11}$ since they highly depend on $n_{9}$. 


\begin{figure}[t]
\centering
\includegraphics[width=0.85\columnwidth]{pics/shared_vs_dedicated_network}
\caption{\label{struct_correlation}Example of structural correlation.}
\vspace{-10pt}
\end{figure}


In various existing virtualization technologies, redundancy is provided in the form of virtual instance replicas, which are ready to takeover the service in case the primary instance fails. Typical solutions like VMware Fault Tolerance~\cite{vmware_ha} or more recent NFV state-of-art system-level frameworks~\cite{kulkarni_reinforce_2018} envision the instantiation of a dedicated backup instance, which runs on a separate node and is kept in synchronization with the primary by logging the incoming traffic. However, such solutions can be resource inefficient as per each NF at least two instances (one primary and one backup) are required to ensure a certain availability level. We exploit the intuitive concept of NF shared reservation for significantly reducing the number of backup NF instances required to satisfy the service requests both in terms of processing capacity and availability demands. 

In the design of CoShare, we exploit these considerations to efficiently use resources and allocate effective backup service function chains.  

}

